Predicting Participation in Cancer Screening Programs with Machine Learning

In this paper, we present machine learning models based on random forest classifiers, support vector machines, gradient boosted decision trees, and artificial neural networks to predict participation in cancer screening programs in South Korea. The top performing model was based on gradient boosted decision trees and achieved an area under the receiver operating characteristic curve (AUC-ROC) of 0.8706 and average precision of 0.8776. The results of this study are encouraging and suggest that with further research, these models can be directly applied to Korea's healthcare system, thus increasing participation in Korea's National Cancer Screening Program.

==> Cancer Screening Participation Prediction/Variable_table.tex <==

    
    
    
	\begin{table}[h]
		\centering
		\resizebox{16cm}{!} {
		\begin{tabular}{|l|l|l|} 
			\hline
			Variable Description & Variable Type \\ [0.5ex] 
			\hline\hline
			 Income Level & Ordinal \\ 
			 \hline
			 Education Level & Ordinal \\
			 \hline
			 Self Perception of Health & Ordinal \\
			 \hline
			 High Blood Pressure Diagnosis & Binary \\
			 \hline
			 Hyperlipidemia Diagnosis  & Binary\\
			 \hline
			 Stroke Diagnosis  & Binary \\
			 \hline
			 Myocardial Infarction/Angina Pectoris Diagnosis & Binary \\
			 \hline
			 Myocardial Infarction Diagnosis & Binary \\
			 \hline
			 Angina Pectoris Diagnosis & Binary \\
			 \hline
			 Arthritis Diagnosis & Binary \\
			 \hline
			 Osteoarthritis Diagnosis & Binary \\
			 \hline
			 Rheumatoid Arthritis Diagnosis & Binary \\
			 \hline
			 Osteoporosis Diagnosis & Binary \\
			 \hline
			 Tuberculosis Diagnosis & Binary \\
			 \hline
			 Asthma Diagnosis & Binary \\
			 \hline
			 Diabetes Diagnosis & Binary \\
			 \hline
			 Thyroid Gland disease Diagnosis & Binary \\
			 \hline
			 Stomach Cancer Diagnosis & Binary \\
			 \hline
			 Liver Cancer Diagnosis & Binary \\
			 \hline
			 Colon Cancer Diagnosis & Binary \\
			 \hline
			 Breast Cancer Diagnosis & Binary \\
			 \hline
			 Cervical Cancer Diagnosis & Binary \\
			 \hline
			 Lung Cancer Diagnosis & Binary \\
			 \hline
			 Thyroid Cancer Diagnosis & Binary \\
			 \hline
			 Other-1 Cancer Diagnosis & Binary \\
			 \hline
			 Other-2 Cancer Diagnosis & Binary \\
			 \hline
			 Depression Diagnosis & Binary \\
			 \hline
			 \end{tabular}
			 \begin{tabular}{|l|l|l|} 
			 Atopic Dermatitis Diagnosis & Binary \\
			 \hline
			 Allergic Rhinitis Diagnosis & Binary \\
			 \hline
			 Sinusitis Diagnosis & Binary \\
			 \hline
			 Otitis Media Diagnosis & Binary \\
			 \hline
			 Cataract Diagnosis & Binary \\
			 \hline
			 Glaucoma Diagnosis & Binary \\
			 \hline
			 Macular Degeneration Diagnosis & Binary \\
			 \hline
			 Renal Failure Diagnosis & Binary \\
			 \hline
			 Hepatitis B Diagnosis & Binary \\
			 \hline
			 Hepatitis C Diagnosis & Binary \\
			 \hline
			 Liver Cirrhosis Diagnosis & Binary \\
			 \hline
			 Influenza Vaccination & Binary \\
			 \hline
			 Regular Health Check-up  & Binary \\
			 \hline
			 Limited Daily/Social Life & Binary \\
			 \hline
			 Employment & Binary \\
			 \hline
			 Self Perception of Stress & Ordinal \\
			 \hline
			 Regular Exercise & Binary \\
			 \hline
			 Nutrition Education Status & Binary \\
			 \hline
			 Private Health Insurance & Binary \\
			 \hline
			 Type of Health Insurance  & Nominal \\
			 \hline
			 Occupation Type & Nominal \\
			 \hline
			 Region & Nominal \\
			 \hline
			 Unmet Healthcare Needs & Nominal \\
			 \hline
			 Causes of Unmet Healthcare Needs & Nominal \\
			 \hline
			 Self Perception of Body Image & Ordinal \\
			 \hline
			 Hospital Admission in Past Year & Binary \\
			 \hline
			 Drinking Level & Ordinal \\
			 \hline
			 Smoking Level & Ordinal \\ [1ex]
			\hline
		\end{tabular}
		}
		\caption{Selected Variables --- Description and Type}
		\label{table:table1}

	\end{table}



==> Variable_table.tex <==

    
    
    
	\begin{table}[h]
		\centering
		\resizebox{16cm}{!} {
		\begin{tabular}{|l|l|l|} 
			\hline
			Variable Description & Variable Type \\ [0.5ex] 
			\hline\hline
			 Income Level & Ordinal \\ 
			 \hline
			 Education Level & Ordinal \\
			 \hline
			 Self Perception of Health & Ordinal \\
			 \hline
			 High Blood Pressure Diagnosis & Binary \\
			 \hline
			 Hyperlipidemia Diagnosis  & Binary\\
			 \hline
			 Stroke Diagnosis  & Binary \\
			 \hline
			 Myocardial Infarction/Angina Pectoris Diagnosis & Binary \\
			 \hline
			 Myocardial Infarction Diagnosis & Binary \\
			 \hline
			 Angina Pectoris Diagnosis & Binary \\
			 \hline
			 Arthritis Diagnosis & Binary \\
			 \hline
			 Osteoarthritis Diagnosis & Binary \\
			 \hline
			 Rheumatoid Arthritis Diagnosis & Binary \\
			 \hline
			 Osteoporosis Diagnosis & Binary \\
			 \hline
			 Tuberculosis Diagnosis & Binary \\
			 \hline
			 Asthma Diagnosis & Binary \\
			 \hline
			 Diabetes Diagnosis & Binary \\
			 \hline
			 Thyroid Gland disease Diagnosis & Binary \\
			 \hline
			 Stomach Cancer Diagnosis & Binary \\
			 \hline
			 Liver Cancer Diagnosis & Binary \\
			 \hline
			 Colon Cancer Diagnosis & Binary \\
			 \hline
			 Breast Cancer Diagnosis & Binary \\
			 \hline
			 Cervical Cancer Diagnosis & Binary \\
			 \hline
			 Lung Cancer Diagnosis & Binary \\
			 \hline
			 Thyroid Cancer Diagnosis & Binary \\
			 \hline
			 Other-1 Cancer Diagnosis & Binary \\
			 \hline
			 Other-2 Cancer Diagnosis & Binary \\
			 \hline
			 Depression Diagnosis & Binary \\
			 \hline
			 \end{tabular}
			 \begin{tabular}{|l|l|l|} 
			 Atopic Dermatitis Diagnosis & Binary \\
			 \hline
			 Allergic Rhinitis Diagnosis & Binary \\
			 \hline
			 Sinusitis Diagnosis & Binary \\
			 \hline
			 Otitis Media Diagnosis & Binary \\
			 \hline
			 Cataract Diagnosis & Binary \\
			 \hline
			 Glaucoma Diagnosis & Binary \\
			 \hline
			 Macular Degeneration Diagnosis & Binary \\
			 \hline
			 Renal Failure Diagnosis & Binary \\
			 \hline
			 Hepatitis B Diagnosis & Binary \\
			 \hline
			 Hepatitis C Diagnosis & Binary \\
			 \hline
			 Liver Cirrhosis Diagnosis & Binary \\
			 \hline
			 Influenza Vaccination & Binary \\
			 \hline
			 Regular Health Check-up  & Binary \\
			 \hline
			 Limited Daily/Social Life & Binary \\
			 \hline
			 Employment & Binary \\
			 \hline
			 Self Perception of Stress & Ordinal \\
			 \hline
			 Regular Exercise & Binary \\
			 \hline
			 Nutrition Education Status & Binary \\
			 \hline
			 Private Health Insurance & Binary \\
			 \hline
			 Type of Health Insurance  & Nominal \\
			 \hline
			 Occupation Type & Nominal \\
			 \hline
			 Region & Nominal \\
			 \hline
			 Unmet Healthcare Needs & Nominal \\
			 \hline
			 Causes of Unmet Healthcare Needs & Nominal \\
			 \hline
			 Self Perception of Body Image & Ordinal \\
			 \hline
			 Hospital Admission in Past Year & Binary \\
			 \hline
			 Drinking Level & Ordinal \\
			 \hline
			 Smoking Level & Ordinal \\ [1ex]
			\hline
		\end{tabular}
		}
		\caption{Selected Variables --- Description and Type}
		\label{table:table1}

	\end{table}



==> Variable_table_2.tex <==

\begin{table}[h]
	    \hspace*{-1cm}
	    \resizebox{13.4cm}{!} {
	    
		\begin{tabular}{|l|l|l|} 
			\hline
			Variable Description & Variable Type \\ [0.5ex] 
			\hline\hline
			 Income Level & Ordinal \\ 
			 \hline
			 Education Level & Ordinal \\
			 \hline
			 Self Perception of Health & Ordinal \\
			 \hline
			 High Blood Pressure Diagnosis & Binary \\
			 \hline
			 Hyperlipidemia Diagnosis  & Binary\\
			 \hline
			 Stroke Diagnosis  & Binary \\
			 \hline
			 \vtop{\hbox{\strut Myocardial Infarction/Angina}\hbox{\strut Pectoris Diagnosis}} & Binary \\
			 \hline
			 Myocardial Infarction Diagnosis & Binary \\
			 \hline
			 Angina Pectoris Diagnosis & Binary \\
			 \hline
			 Arthritis Diagnosis & Binary \\
			 \hline
			 Osteoarthritis Diagnosis & Binary \\
			 \hline
			 Rheumatoid Arthritis Diagnosis & Binary \\
			 \hline
			 Osteoporosis Diagnosis & Binary \\
			 \hline
			 Tuberculosis Diagnosis & Binary \\
			 \hline
			 Asthma Diagnosis & Binary \\
			 \hline
			 Diabetes Diagnosis & Binary \\
			 \hline
			 Thyroid Gland disease Diagnosis & Binary \\
			 \hline
			 Stomach Cancer Diagnosis & Binary \\
			 \hline
			 Liver Cancer Diagnosis & Binary \\
			 \hline
			 Colon Cancer Diagnosis & Binary \\
			 \hline
			 Breast Cancer Diagnosis & Binary \\
			 \hline
			 Cervical Cancer Diagnosis & Binary \\
			 \hline
			 Lung Cancer Diagnosis & Binary \\
			 \hline
			 Thyroid Cancer Diagnosis & Binary \\
			 \hline
			 Other-1 Cancer Diagnosis & Binary \\
			 \hline
			 Other-2 Cancer Diagnosis & Binary \\
			 \hline
			 Depression Diagnosis & Binary \\
			 \hline
		\end{tabular}


			 \begin{tabular}{|l|l|l|} 
			 Atopic Dermatitis Diagnosis & Binary \\
			 \hline
			 Allergic Rhinitis Diagnosis & Binary \\
			 \hline
			 Sinusitis Diagnosis & Binary \\
			 \hline
			 Otitis Media Diagnosis & Binary \\
			 \hline
			 Cataract Diagnosis & Binary \\
			 \hline
			 Glaucoma Diagnosis & Binary \\
			 \hline
			 Macular Degeneration Diagnosis & Binary \\
			 \hline
			 Renal Failure Diagnosis & Binary \\
			 \hline
			 Hepatitis B Diagnosis & Binary \\
			 \hline
			 Hepatitis C Diagnosis & Binary \\
			 \hline
			 Liver Cirrhosis Diagnosis & Binary \\
			 \hline
			 Influenza Vaccination & Binary \\
			 \hline
			 Regular Health Check-up  & Binary \\
			 \hline
			 Limited Daily/Social Life & Binary \\
			 \hline
			 Employment & Binary \\
			 \hline
			 Self Perception of Stress & Ordinal \\
			 \hline
			 Regular Exercise & Binary \\
			 \hline
			 Nutrition Education Status & Binary \\
			 \hline
			 Private Health Insurance & Binary \\
			 \hline
			 Type of Health Insurance  & Nominal \\
			 \hline
			 Occupation Type & Nominal \\
			 \hline
			 Region & Nominal \\
			 \hline
			 Unmet Healthcare Needs & Nominal \\
			 \hline
			 Causes of Unmet Healthcare Needs & Nominal \\
			 \hline
			 Self Perception of Body Image & Ordinal \\
			 \hline
			 Hospital Admission in Past Year & Binary \\
			 \hline
			 Drinking Level & Ordinal \\
			 \hline
			 Smoking Level & Ordinal \\ [1ex]
			\hline
		\end{tabular}
        }
		\caption{Selected Variables --- Description and Type}
		\label{table:table1}

	\end{table}
